Proof-of-Turn: Blockchain consensus using a round-robin procedure as one possible solution for cutting costs in mobile games

This master thesis deals with Blockchain Technology in mobile turn based peer to peer games. First, it investigates the capabilities of Blockchain Technology to be used for gaming applications. In this regard, among others, Proof-of-Mechanisms, Vote-based Consensus and several Performance Improvements are described. Second, several smart contracts are introduced to show the general feasibility of turn based games hosted on Blockchain Technology. More specific, Hidden transactions, Randomization, Piles of Cards, Fog of War elements, Data allocation improvements and other smart contracts are specified. Third, a special Proof-of-Turn consensus mechanism, based on the Blockchain Technology, is defined to enable game publishers to cut costs in the means of their provided game servers. Herein, Byzantine Fault Tolerance, Peering, the CAP Theorem, Interoperability among other characteristics are covered. Last, these measures shall additionally raise the trust level among the players in mobile turn based games.

==> CHANGELOG <==
The version number of all files is changed for every release. Please refer to the details below in order to see which files were changed.

2021/02/22 v1.7.1
* [udesoftec-bibcommon.sty] fixing \bbldoi by switching to pkg:uri
* [udesoftec.cls] re-enabled auto-output of glossary if existing
* [udesoftec.cls] add pkg:bookmark to replace bookmarks from pkg:hyperref
* [udesoftec-biblatex.sty] fix deprecated extrayear
* [udesoftec-bibcommon.sty] fix deprecated \ifnumber
* [udesoftec.cls] remove supervisor from example front page
* [udesoftec.cls] remove deprecationwarnings for \clearscr*

2020/03/09 v1.6.6
* [udesoftec.cls] fix confidentially clause
* improve build steps for package, linting of files

2018/06/20 v1.6.5 (unreleased)
* internal changes
 
2018/04/24 v1.6.4 (unreleased)
* [udesoftec.cls] fix statutory declaration
* [udesoftec.cls] list of abbreviations should have more indent due to longer abbreviations
 
2018/04/02 v1.6.3
* [udesoftec-biblatex.sty] fix regression with duplicate bibliography toc entry

2018/03/28 v1.6.2
* [udesoftec-biblatex.sty] Corrected headline showing last chapter instead of bibliography
* [udesoftec.cls] fixed german heading for list of abbreviations
* [udesoftec-doc.pdf] corrected TeXnicCenter Configuration
* Bumping version number
 
2017/12/08 v1.6.1 (unreleased)
* Internal fixes due to new build tool
* Bumping version number
 
2017/05/12 v1.6.0
* Internal fixes due to new build tool
* [udesoftec.cls] removing PDF warnings
* [udesoftec-biblatex.sty] new compatibility with biblatex>3.5 new naming scheme
* [udesoftec.cls] fixed list of abbreviations
* [udesoftec.bst] fixed compatibility issue with MikTeX
* [udesoftec.bst] fixed issue with @incollection missing volume argument resulting in error
* [udesoftec.bst] removed url+urldate from output if DOI is present
* [udesoftec.bst] fixed issue with @article which has month set resulting in warning
 
2016/08/15 v1.5.5
* [udesoftec.cls] fixed cover page to fit new exam regulations
* [udesoftec.cls] fixed bug resulting in xpatch errors due to koma update
* [udesoftec.cls] added template version to English cover page
* [udesoftec-biblatex.sty] updated deprecated code for new biblatex
 
2015/09/28 v1.5.4 (unreleased)
* [udesoftec-biblatex.sty] fixed references heading wrong label and missing toc entry
* [udesoftec-biblatex.sty] fixed bbl for @incollection
* [udesoftec-biblatex.sty] changed bbl to raggedright and set bibhang to 1.5em
* [udesoftec-biblatex.sty] some bbl spaces are now non-breaking spaces to improve word-wrap
* [udesoftec-bst.sty] changed bbl to raggedright and set bibhang to 1.5em
* [udesoftec-bst.sty] some bbl spaces are now non-breaking spaces to improve word-wrap
 
2015/09/04 v1.5.3 (unreleased)
* [udesoftec-doc.pdf] corrected package dependencies
* [udesoftec-biblatex.sty] fixed incompatibility with \citemulti from udesoftec-bibcommon
* [udesoftec-biblatex.sty] fixed incompatibility with \citequotepar from udesoftec-bibcommon
* [udesoftec-biblatex.sty] defaulting \cite to \citep for compatibility with udesoftec-bst
* [udesoftec.cls] changed quotation style
 
2015/09/04 v1.5.2
* [udesoftec.cls] Regression: \acadmicfield was dropped from default title page
* [udesoftec.bst] repaired doi error parsing
* [udesoftec-bibcommon.sty] automatic prefixing of pages for BibTeX: if page is numeric add prefix, else use string supplied instead of page, e.g. \cite[43-56]{Bib} for citing "pp. 42-56" and \cite[B.2]{Bib} to cite "B.2" of a document without pages. In order to reproduce old behavior use: \renewcommand*{\bblInTextPagePrefix}[1]{}
 
2015/08/27 v1.5.1
* Improving interop between BibTeX and BibLaTeX styles
* [udesoftec-biblatex.sty] adapting formating to remove major bugs  
* [udesoftec.cls] switching class mapping of "en" to "british" instead of "english" for better date representation
 
2015/08/25 v1.5.0 (unreleased)
* Big code sprint and bugfixing!
* [udesoftec.bst] fixed order of elements in biblography
* [udesoftec.cls] major cleanup and reordering of cls file
* [udesoftec-bst.sty] fixed wrong font size after first ISBN/ISSN in bibliography
* NEW [udesoftec-biblatex.sty] adding basic support in the architecture of the class for biblatex. Currently the citations are barely how they should look like and the package is highly experimental.
* NEW [udesoftec-bibcommon.sty] provide basic support for bibtex/bst and biber/bbx/biblatex to use the same commands for design of citations and bibliography, will be included automatically by udesoftec-bst and udesoftec-biblatex
* [udesoftec-bibcommon.sty] provide support for reformating the dates in bibliography for urldate or techstandards. Dates should have the format "yyyy-mm-dd" or "dd.mm.yyyy". A bit of robustness is coded in, due to different exports having different date formats. In case you run into errors, feel free to report your date format.
* [udesoftec-bibcommon.sty] changed punctuation for more fit towards Springer Basic
* [udesoftec-bibcommon.sty] fixed some citations not having \textsc set
 
2015/08/20 v1.4.8
* [udesoftec.bst] fixing regression introduced in 1.4.7 with some cite commands preventing year from being placed in text

2015/08/19 v1.4.7
* [udesoftec-doc] fixed documentation for package depencies due to used packages being updated
* [udesoftec.cls] removed deprecated fixltx2e
* [udesoftec.bst] added new doctype @techstandard for better interop with Citavi and standards, refer to documentation for further details
* [udesoftec.bst] fixed a problem with Citavi BibTeX exports having a {\textunderscore } in doi
* [udesoftec.cls] added new command \citemulti{}

2015/05/14 v1.4.6
* replaced AtBeginDocument with AtEndPreamble for better interop with other packages
* changed page margin to fit better to new font and improve readability on 4:3 tablets as well as paper while marginnotes get less space

2014/11/10 v1.4.5
* fixed list of abbreviations not being created

2014/08/23 v1.4.4
* [udesoftec-extra.sty] removed detokenize from DOI in bibtex (due to Citavi adding tokens to bibtex exports).
* [udesoftec-bst.sty] corrected spacing between edition ordinal and label

2014/07/16 v1.4.3 (unreleased)
* [udesoftec.cls] corrected auto-detection of list-of-acronyms, because sometimes a blank page was created if acronyms where defined but none was used.
* [udesoftec.cls] added udesoftec version to default output of version on titlepage for easier reference by students
* [udesoftec-bst.sty] added option for page prefix of in-text-citations (e.g. to switch easily between German 'S.' and English 'p')
* [udesoftec-extra.sty] added page prefix for in-text-citations '\bblp' - doesn't use 'pp' for multiple pages.
* [udesoftec-extra.sty] removed detokenize from DOI in bibtex (due to Citavi adding tokens to bibtex exports).

2014/06/22 v1.4.2
* [udesoftec-doc.pdf] created an rss feed for udesoftec updates and added it to documentation
* [udesoftec.cls] added auto-detection to list-of-* to just generate them if needed. So the omit-*-Options are in most cases unnecessary, but will still work in order to override the detection.

2014/05/27 v1.4.1
* minor improvements to documentation
* moved tested addtitions from udesoftec-extra.sty to udesoftec.cls

2014/05/19 v1.4.0
* splitted documentclass in two files to create udesoftec-bst.sty which holds the configuration for bibstyle and might be used separately
* major code cleanup: removed many usepackages and configuration which is not necessary anymore
* major documentation cleanup and improvement: added list of listings for easy access to code examples
* added list of listings and classoption "omit-lol"
* improved the title page background files
* updated tlmgr install for new dependencies 
* fixed font usage to just stick to one family
* changed line spacing to a more appropiate value.
* changed box size to be same for all kind of boxes (e.g. citequotepar, lstlisting)

== WARNING: your document might need update using newer version ==

2014/05/13 v1.3.8
* corrected some URLs in source
* changed default chapter design (e.g. used by list-of-*)
* added abstract with document options omit-a and long-a
* added more documentation about enumerations
* added chapter numbering, document title and toc to pdf bookmarks
* changed pdf bookmarks to be open for 2 levels
* corrected list of abbreviations design
* corrected some wrong ordering of usepackage
* changed quotebox environment to not break pages due to current problems with them using the same space as figure

2014/04/30 v1.3.7
* removed deprecated page layout combinations and thus removed complex page layout creation to fall back to KOMA defaults (thx to pointing this out unknown phone caller).
* added default binding correction (BCOR) for print layout
* major cleanup of class structure
* fixed confidentially clause

2014/04/14 v1.3.6
* fixed problems with combination of cls-options 'proposal' and 'final'
* fixed problem when no layout was chosen
* fixed missing inlinetodo-command for option 'omit-todo'

2014/04/07 v1.3.5
* added document option 'proposal' which equals all omit-*
* corrected English version of confidentially clause
* set default layout to 'screen'
* omit warning if no layout chosen
* corrected cls version number and date format
* corrected combinations of options vawi* and en overriding default labels on titlepage 

2014/03/31 v1.3.4
* added option omit-toc for research proposals
* documentation changes
** english summary updated
** minor changes to sectioning and labels
** updated link to example document
** added additional packages to tlmgr command to support OSX BasicTeX

2014/03/11 v1.3.3
* added statutory declaration to document (omit with 'omit-sd')

2014/02/18 v1.3.2
* fixed broken CRLF terminated line endings
* corrected URLs for CTAN mirror use

2014/02/18 v1.3.1
* repaired option _vawibamberg_ in combination with option _en_
* changed document configuration options like \def \entitle{my english title} to non-def commands like \title or \author

2014/01/10 v1.3.0
* switched from package expdlist to enumitem: description environment options need to be changed!

== WARNING: document might need update using newer version ==

2013/08/14 v1.2.1
* fixed misconfigured line endings and zip format

2013/08/14
* added udesoftec.tds.zip to support other TeX Collections
* removed problem with umlauts in lstlisting-env
* added (currently emtpy) udesoftec-extra.sty, for easier updating in case of changed behaviour
* improved documentation
* improved \parExample and \citequotepar
* added classoption omit-loa
* added classoption omit-todos
* added \printglossaries, \printacronyms and \listoftodos to \AtBeginDocument and \AtEndDocument for convenience (i.e. they aren't necessary in the document anymore)
* made \listoftodos conditional
* correct bibstyle "lastaccessed" format
* added additional sections to manual with more examples
* english cover wasn't found due to wrong filename referenced
* option for confidentially clause now available

2013/07/09
* added version number
* updated cover page line spacing
* updated README and added instruction for cover files
* added packages listings, multicol and verbatim
* updated documentation
** added English abstract
** better outline to improve understanding
** included package listing
*** included FAQ entry for problems with cover files

2013/06/28
* better filenames
* update to udesoftec-cover-uba.pdf: smaller filesize and undamaged PDF file

2013/06/26 
* Initial CTAN Upload


==> contents/C_B_Meta.tex <==


\addcontentsline{toc}{section}{Abstract}
\section*{Abstract}
\label{sec:Abstract}

\textbf{TL;DR}: blah \\

This master thesis deals with Blockchain Technology in turn based online peer to peer games. \\

This thesis argues(/shows) that a distributed database, based on the Blockchain technology, is capable to enable game publishers to cut costs in the means of running servers, whilst raising the trust level among the players in tunr based games. \\



\addcontentsline{toc}{section}{Preamble}
\section*{Preamble}
\label{sec:Preamble}
The following definitions are probably known by the reader, nevertheless they are given beforehand for a better reading experience and an improved understanding:
\begin{enumerate}
	\item \textbf{Blockchain Technology} \label{def:BCT} \\
	\textit{Blockchain Technology} (\textbf{BCT}) ".. is a form of distributed ledger technology, deployed on a peer-to-peer network where all data are replicated, shared, and synchronously spread across multiple peers. The technology allows actors participating in the network to perform, sign, and announce transactions by employing public key cryptography. Transactions are executed following a consensus protocol operated by specific nodes to ensure the validity of transactions requested by other peers in the network, and to synchronize all shared copies of the distributed ledger. During a consensus protocol execution, the data of valid transactions, along with other required metadata concerning the network, and the hash of the previous block are bundled into a block using hashing functions. The essential and key property reflecting \hyperref[def:BCT]{BCT} architectures is that each block contains the hash of their predecessor, therefore linking all prior transactions to newly appended transactions; the blocks therefore form a chain with the aim of establishing a tamper-proof historical record"
	\cite[13]{Butijn.2020} \\
	Further details can be found in the chapter \hyperref[sec:BlockchainTech]{Blockchain Technology}.
	
	\item \textbf{Cheating}	\label{def_Cheating} \\
	Illegal behavior, which leads to an advantage for the cheating person.
	Although the rules of the game shall prevent such behavior, the cheating person found a way to circumvent the game mechanics.
	
	\item \textbf{Cryptocurrency} \label{def_Cryptocurrency} \\
	A cryptocurrency is a construct of hypothetical value - just  as any other currency - but it is not governed by a central institution but rather by a distributed algorithm.
	The transactions are secured by cryptographic functions as well as mathematical problems.
	
	\item \textbf{Dark Patterns} \label{def_DarkPatterns} \\
	Mechanics withing games which nudge players, more or less obtrusive, to behave in a specific way.
	If a player gives in to the intrusiveness, a (hidden) negative or neutral consequence follows.
	\hyperref[def_DarkPatterns]{Dark patterns} are seen as malicious mechanics by the publishers.
	
	\item \textbf{Gamers, Players, Peers and Nodes} \label{def_GamersPlayersPeersAndNodes} \\
	Although in other context gamers, players, peers and nodes could be seen as synonymous, here they need to be distinguished.
	A node will be considered as a hardware system, which is part of a (gaming-)network.
	Players are in game character, who are controlled by gamers.
	Gamers are persons, who e.g. own nodes.
	Finally, peers are persons, who can be gamers but predominantly own or maintain a node.
	
	\item \textbf{Genesis Block} \label{def_GenesisBlock} \\
	The \hyperref[def_GenesisBlock]{genesis block} ".. is the first block in the chain and has a predetermined hash" \cite[181]{Oliveira.19.02.201921.02.2019}.
	
	\item \textbf{Mining} \label{def_Mining} \\
	The process of solving a computational hard mathematical puzzle by finding the right nonce (a random number) for the block-header based on information of the prior block.
	The nodes executing the calculations are referred to as miners in the \hyperref[def_Cryptocurrency]{Cryptocurrencies} nomenclature.
	The first miner to finish creates the next block and is rewarded by receiving an amount of the underlying \hyperref[def_Cryptocurrency]{Cryptocurrency} (BUTIJN, p. 60, 2020). (???)
	
	\item \textbf{Principal-Agent Problem} \label{def_PrincipalAgentProblem} \\
	"The principal-agent literature is concerned with how one individual, the principal (say an employer), can design a compensation system (a contract) which motivates another individual, his agent (say the employee), to act in the principal's interests" (Stiglitz, p. 241, 1989).
	
	\item \textbf{Transactions and Smart Contracts} \label{def_TransactionsAndSC} \\
	Every entry in a Blockchain is considered a transaction.	
	If data in a transaction is constraint to a set of rules, the transaction is called a Smart Contract (SC).
	
	\item \textbf{Trolling} \label{def_Trolling} \\
	Trolling in online communities can either be cheating or malicious/hostile behavior. 
	
\end{enumerate}

==> contents/C_G_Outlook.tex <==






